InstantEmbedding: Efficient Local Node Representations

In this paper, we introduce InstantEmbedding, an efficient method for generating single-node representations using local PageRank computations. We theoretically prove that our approach produces globally consistent representations in sublinear time. We demonstrate this empirically by conducting extensive experiments on real-world datasets with over a billion edges. Our experiments confirm that InstantEmbedding requires drastically less computation time (over 9,000 times faster) and less memory (by over 8,000 times) to produce a single node's embedding than traditional methods including DeepWalk, node2vec, VERSE, and FastRP. We also show that our method produces high quality representations, demonstrating results that meet or exceed the state of the art for unsupervised representation learning on tasks like node classification and link prediction.

==> data/data.orkut.epsilon.tex <==




















==> figures/fig.memory-multifig.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
    \begin{groupplot}[
      group style={
        group name=heaptrack,
        group size=2 by 1,
        horizontal sep=2cm,
      },
      width=4.5cm,
      height=3.5cm,
    %   ymode=log,
    %   xmode=log,
      ymajorgrids=true,
      grid style=dotted,
    ]
    % Chart for Nodes-to-Runtime
    \nextgroupplot[xlabel={(a) |V|},
                   ymode=log,
                   xmode=log,
                   ylabel={\small Memory Used (MB)}
                   ]
        \addplot[color=customgreen, only marks, mark=triangle*] coordinates {
            (3890, 0.13344) % HomoSapiens
            (4777, 0.364860) % POS
            (10312, 0.520870) % BlogCatalog
            (44034, 0.188130) % AcademicConfs
            (51821, 0.135920) % AcademicCOA
            (80513, 0.286710) % Flickr
            (1138499, 1.010000) % YouTube
            (2449029, 0.743090) % Amazon2M
            (3072441, 7.78) % Orkut
            % (65608366, 9.5) % Friendster ---- TBD
        };
        \label{method:InstantEmbedding}
        \addplot[color=customblue, only marks, mark=pentagon*] coordinates {
            (3890, 16.75) % HomoSapiens
            (4777, 20.92) % POS
            (10312, 46.21) % BlogCatalog
            (44034, 187.54) % AcademicConfs
            (51821, 220.32) % AcademicCOA
            (80513, 387.67) % Flickr
            (1138499, 4860.00) % YouTube
            (2449029, 10910.00) % Amazon2M ---- TBD
            (3072441, 14000.00) % Orkut ---- TBD
            % (65608366, 28000.00) % Friendster ---- TBD
        };
        \label{method:DeepWalk}
        \addplot[color=customred, only marks, mark=diamond*] coordinates {
            (3890, 8.39) % HomoSapiens
            (4777, 10.64) % POS
            (10312, 23.92) % BlogCatalog
            (44034, 92.01) % AcademicConfs
            (51821, 107.85) % AcademicCOA
            (80513, 212.50) % Flickr
            (1138499, 2360.00) % YouTube
            (2449029, 5520.00) % Amazon2M
            (3072441, 7240.00) % Orkut
            % (65608366, 14480.00) % Friendster ---- TBD
        };
        \label{method:VERSE}
        \addplot[color=customyellow, only marks, mark=oplus*] coordinates {
            (3890, 65.98) % HomoSapiens
            (4777, 816.66) % POS
            (10312, 3000.00) % BlogCatalog
            (44034, 284.20) % AcademicConfs
            (51821, 279.75) % AcademicCOA
            (80513, 70110.00) % Flickr
            (1138499, 28410.00) % YouTube
            % (2449029, 0) % Amazon2M
            % (3072441, 1) % Orkut
            % (65608366, 696888) % Friendster ---- TBD
        };
        \label{method:Node2Vec}
        \addplot[color=customgrey, only marks, mark=square*] coordinates {
            (3890, 197.67) % HomoSapiens
            (4777, 245.52) % POS
            (10312, 504.65) % BlogCatalog
            (44034, 1660.00) % AcademicConfs
            (51821, 1770.00) % AcademicCOA
            (80513, 3830.00) % Flickr
            (1138499, 40610.00) % YouTube
            (2449029, 125870.00) % Amazon2M
            % (3072441, 20) % Orkut
            % (65608366, 696888) % Friendster ---- TBD
        };
        \label{method:FastRP}
    
    
    % Chart for Edges-to-Runtime
    \nextgroupplot[xlabel={(b) |E|},
                   ymode=log,
                   xmode=log
                   ]
        \addplot[color=customgreen, only marks, mark=triangle*] coordinates {
            (38292, 0.13344) % HomoSapiens
            (92406, 0.364860) % POS
            (195361, 0.188130) % AcademicConfs
            (333983, 0.520870) % BlogCatalog
            (355926, 0.135920) % AcademicCOA
            (2990443, 1.010000) % YouTube
            (5899882, 0.286710) % Flickr
            (61859076, 0.743090) % Amazon2M
            (117185083, 7.78) % Orkut
            % (1806067135, 9.5) % Friendster ---- TBD
        };
        \label{method:InstantEmbedding}
        \addplot[color=customblue, only marks, mark=pentagon*] coordinates {
            (38292, 16.75) % HomoSapiens
            (92406, 20.92) % POS
            (195361, 187.54) % AcademicConfs
            (333983, 46.21) % BlogCatalog
            (355926, 220.32) % AcademicCOA
            (2990443, 4860.00) % YouTube
            (5899882, 387.67) % Flickr
            (61859076, 10910.00) % Amazon2M ---- TBD
            (117185083, 14000.00) % Orkut ---- TBD
        };
        \label{method:DeepWalk}
        \addplot[color=customred, only marks, mark=diamond*] coordinates {
            (38292, 8.39) % HomoSapiens
            (92406, 10.64) % POS
            (195361, 92.01) % AcademicConfs
            (333983, 23.92) % BlogCatalog
            (355926, 107.85) % AcademicCOA
            (2990443, 2360.00) % YouTube
            (5899882, 212.50) % Flickr
            (61859076, 5520.00) % Amazon2M
            (117185083, 7240.00) % Orkut ---- TBD
        };
        \label{method:VERSE}
        \addplot[color=customyellow, only marks, mark=oplus*] coordinates {
            (38292, 65.98) % HomoSapiens
            (92406, 816.66) % POS
            (195361, 284.20) % AcademicConfs
            (333983, 3000.00) % BlogCatalog
            (355926, 279.75) % AcademicCOA
            (2990443, 28410.00) % YouTube
            (5899882, 70110.00) % Flickr
            % (61859076, 0) % Amazon2M
            % (117185083, 1) % Orkut
            % (1806067135, 0.5) % Friendster ---- TBD
        };
        \label{method:Node2Vec}
        \addplot[color=customgrey, only marks, mark=square*] coordinates {
            (38292, 197.67) % HomoSapiens
            (92406, 245.52) % POS
            (195361, 1660.00) % AcademicConfs
            (333983, 504.65) % BlogCatalog
            (355926, 1770.00) % AcademicCOA
            (2990443, 40610.00) % YouTube
            (5899882, 3830.00) % Flickr
            (61859076, 125870.00) % Amazon2M
            % (117185083, 20) % Orkut
            % (1806067135, 0.5) % Friendster ---- TBD
        };
        \label{method:FastRP}
    
    
    % Chart for % Increase in Memory.
    % \nextgroupplot[xlabel={(c) Embedding Size},
    %               symbolic x coords={64,128,256,512},
    %               xtick={64,128,256,512},
    %               ylabel={\small Avg \% Increase},
    %               xshift=2em
    %               ]
    %     \addplot[color=customgreen, mark=triangle*, thick] coordinates {
    %         (64, 0)
    %         (128, 0)
    %         (256, 0)
    %         (512, 0)
    %     };
    %     \label{method:InstantEmbedding}
    %     \addplot[color=customblue, mark=pentagon*, thick] coordinates {
    %         (64, 0)
    %         (128, 63.552)
    %         (256, 171.615)
    %         (512, 445.435)
    %     };
    %     \label{method:DeepWalk}
    %     \addplot[color=customred, mark=diamond*, thick] coordinates {
    %         (64, 0)
    %         (128, 63.843)
    %         (256, 191.357)
    %         (512, 447.125)
    %     };
    %     \label{method:VERSE}
    %     \addplot[color=customyellow, mark=oplus*, thick] coordinates {
    %         (64, 0)
    %         (128, 7.566)
    %         (256, 22.659)
    %         (512, 52.840)
    %     };
    %     \label{method:Node2Vec}
    %     \addplot[color=customgrey, mark=square*, thick] coordinates {
    %         (64, 0)
    %         (128, 75.647)
    %         (256, 227.274)
    %         (512, 538.528)
    %     };
    %     \label{method:FastRP}
    \end{groupplot}

    % global ylabel
    % \path (current bounding box.west)-- node[anchor=south,rotate=90,align=center] 
    %     {\tiny Memory Used (MB)} (current bounding box.west);
    % global xlabel
    % \node[below = 0.1cm of current bounding box.south] {Embedding Size};

    % legend
    \path (current bounding box.north)-- coordinate(legendpos)
        (current bounding box.north);
    \matrix[matrix of nodes,
            anchor=south,
            draw,
            inner sep=0.2em,
            draw,
            font=\small]
            at(legendpos)
            {
                \ref{method:InstantEmbedding} & InstantEmbed &[5pt]
                \ref{method:DeepWalk} & DeepWalk &[5pt]
                \ref{method:Node2Vec} & node2vec &[5pt]
                \ref{method:VERSE} & VERSE &[5pt]
                \ref{method:FastRP} & FastRP &[5pt] \\
            };
\end{tikzpicture}
\caption{Memory consumption required per method to generate a 512-size node embedding per (a) number of vertices in the graph |V| and (b) number of undirected edges in the graph |E|.}
\label{fig:heaptrack}
\end{figure}

==> figures/fig.running-time-multifig.tex <==
\todo{Filipe: best-fit lines}
\begin{figure}[t]
\centering
\begin{tikzpicture}
    \begin{groupplot}[
      group style={
        group name=runtimeplots,
        group size=3 by 1,
        % horizontal sep=1.5cm,
      },
      width=4.5cm,
      height=3.5cm,
    %   ymode=log,
    %   xmode=log,
      ymajorgrids=true,
      grid style=dotted,
    ]
    
    % Chart for Nodes-to-Runtime
    \nextgroupplot[xlabel={(a) |V|},
                   ymode=log,
                   xmode=log,
                   ylabel={\small Running Time  (s)}
                   ]
        \addplot[color=customgreen, only marks, mark=triangle*] coordinates {
            (3890, 0.009) % HomoSapiens
            (4777, 0.009) % POS
            (10312, 0.04) % BlogCatalog
            (44034, 0.009) % AcademicConfs
            (51821, 0.009) % AcademicCOA
            (80513, 0.10) % Flickr
            (1138499, 0.08) % YouTube
            (2449029, 0.16) % Amazon2M
            (3072441, 0.16) % Orkut
            % (65608366, 0.30) % Friendster ---- TBD
        };
        \label{method:InstantEmbedding}
        \addplot[color=customblue, only marks, mark=pentagon*] coordinates {
            (3890, 257.36) % HomoSapiens
            (4777, 366.14) % POS
            (10312, 677.98) % BlogCatalog
            (44034, 2766.94) % AcademicConfs
            (51821, 3557.95) % AcademicCOA
            (80513, 5978.61) % Flickr
            (1138499, 8127520) % YouTube
            (2449029, 174222.96) % Amazon2M ---- TBD
            (3072441, 348444) % Orkut ---- TBD
            % (65608366, 696888) % Friendster ---- TBD
        };
        \label{method:DeepWalk}
        \addplot[color=customred, only marks, mark=diamond*] coordinates {
            (3890, 105.49) % HomoSapiens
            (4777, 102.52) % POS
            (10312, 199.00) % BlogCatalog
            (44034, 864.84) % AcademicConfs
            (51821, 1028.13) % AcademicCOA
            (80513, 1874.51) % Flickr
            (1138499, 31091.85) % YouTube
            (2449029, 74322.51) % Amazon2M
            (3072441, 89257.62) % Orkut ---- TBD
            % (65608366, 178514) % Friendster ---- TBD
        };
        \label{method:VERSE}
        \addplot[color=customyellow, only marks, mark=oplus*] coordinates {
            (3890, 24.85) % HomoSapiens
            (4777, 28.91) % POS
            (10312, 67.86) % BlogCatalog
            (44034, 281.62) % AcademicConfs
            (51821, 328.46) % AcademicCOA ---- TBD
            (80513, 831.01) % Flickr
            (1138499, 7492.15) % YouTube
            % (2449029, 0) % Amazon2M
            % (3072441, 1) % Orkut
            % (65608366, 696888) % Friendster ---- TBD
        };
        \label{method:Node2Vec}
        \addplot[color=customgrey, only marks, mark=square*] coordinates {
            (3890, 1.80) % HomoSapiens
            (4777, 2.20) % POS
            (10312, 5.24) % BlogCatalog
            (44034, 5.77) % AcademicConfs
            (51821, 4.91) % AcademicCOA
            (80513, 73.19) % Flickr
            (1138499, 82.11) % YouTube
            (2449029, 909.86) % Amazon2M
            % (3072441, 20) % Orkut
            % (65608366, 696888) % Friendster ---- TBD
        };
        \label{method:FastRP}
    
    
    % Chart for Edges-to-Runtime
    \nextgroupplot[xlabel={(b) |E|}, 
                   ymode=log,
                   xmode=log,
                   xshift=-.5em
                   ]
        \addplot[color=customgreen, only marks, mark=triangle*] coordinates {
            (38292, 0.009) % HomoSapiens
            (92406, 0.009) % POS
            (195361, 0.009) % AcademicConfs
            (333983, 0.04) % BlogCatalog
            (355926, 0.009) % AcademicCOA
            (2990443, 0.08) % YouTube
            (5899882, 0.10) % Flickr
            (61859076, 0.16) % Amazon2M
            (117185083, 0.16) % Orkut
            % (1806067135, 0.30) % Friendster ---- TBD
        };
        \label{method:InstantEmbedding}
        \addplot[color=customblue, only marks, mark=pentagon*] coordinates {
            (38292, 257.36) % HomoSapiens
            (92406, 366.14) % POS
            (195361, 2766.94) % AcademicConfs
            (333983, 677.98) % BlogCatalog
            (355926, 3557.95) % AcademicCOA
            (2990443, 8127520) % YouTube
            (5899882, 5978.61) % Flickr
            (61859076, 174222.96) % Amazon2M ---- TBD
            (117185083, 348444) % Orkut ---- TBD
        };
        \label{method:DeepWalk}
        \addplot[color=customred, only marks, mark=diamond*] coordinates {
            (38292, 105.49) % HomoSapiens
            (92406, 102.52) % POS
            (195361, 864.84) % AcademicConfs
            (333983, 199.00) % BlogCatalog
            (355926, 1028.13) % AcademicCOA
            (2990443, 31091.85) % YouTube
            (5899882, 1874.51) % Flickr
            (61859076, 74322.51) % Amazon2M
            (117185083, 89257.62) % Orkut ---- TBD
        };
        \label{method:VERSE}
        \addplot[color=customyellow, only marks, mark=oplus*] coordinates {
            (38292, 24.85) % HomoSapiens
            (92406, 28.91) % POS
            (195361, 281.62) % AcademicConfs
            (333983, 67.86) % BlogCatalog
            (355926, 328.46) % AcademicCOA ---- TBD
            (2990443, 7492.15) % YouTube
            (5899882, 831.01) % Flickr
            % (61859076, 0) % Amazon2M
            % (117185083, 1) % Orkut
            % (1806067135, 0.5) % Friendster ---- TBD
        };
        \label{method:Node2Vec}
        \addplot[color=customgrey, only marks, mark=square*] coordinates {
            (38292, 1.80) % HomoSapiens
            (92406, 2.20) % POS
            (195361, 5.77) % AcademicConfs
            (333983, 5.24) % BlogCatalog
            (355926, 4.91) % AcademicCOA
            (2990443, 82.11) % YouTube
            (5899882, 73.19) % Flickr
            (61859076, 909.86) % Amazon2M
            % (117185083, 20) % Orkut
            % (1806067135, 0.5) % Friendster ---- TBD
        };
        \label{method:FastRP}
    
    
    % Chart for % Increase in latency.
    \nextgroupplot[xlabel={(c) Embedding Size},
                   symbolic x coords={64,128,256,512},
                   xtick={64,128,256,512},
                   ylabel={\small Avg \% Increase},
                   xshift=2em
                   ]
        \addplot[color=customgreen, mark=triangle*, thick] coordinates {
            (64, 0)
            (128, 0)
            (256, 0)
            (512, 0)
        };
        \label{method:InstantEmbedding}
        \addplot[color=customblue, mark=pentagon*, thick] coordinates {
            (64, 0)
            (128, 69.859)
            (256, 180.283)
            (512, 338.969)
        };
        \label{method:DeepWalk}
        \addplot[color=customred, mark=diamond*, thick] coordinates {
            (64, 0)
            (128, 31.945)
            (256, 83.270)
            (512, 148.052)
        };
        \label{method:VERSE}
        \addplot[color=customyellow, mark=oplus*, thick] coordinates {
            (64, 0)
            (128, 14.301)
            (256, 47.776)
            (512, 107.826)
        };
        \label{method:Node2Vec}
        \addplot[color=customgrey, mark=square*, thick] coordinates {
            (64, 0)
            (128, 29.203)
            (256, 69.089)
            (512, 155.439)
        };
        \label{method:FastRP}
    \end{groupplot}

    % global ylabel
    % \path (current bounding box.west)-- node[anchor=south,rotate=90,align=center] 
    %     {Running time (s)} (current bounding box.west);

    % global xlabel
    % \node[below = 0.1cm of current bounding box.south] {Embedding Size};

    % legend
    \path (current bounding box.north)-- coordinate(legendpos)
        (current bounding box.north);
    \matrix[matrix of nodes,
            anchor=south,
            draw,
            inner sep=0.2em,
            draw,
            font=\small]
            at(legendpos)
            {
                \ref{method:InstantEmbedding} & InstantEmbed &[5pt]
                \ref{method:DeepWalk} & DeepWalk &[5pt]
                \ref{method:Node2Vec} & node2vec &[5pt]
                \ref{method:VERSE} & VERSE &[5pt]
                \ref{method:FastRP} & FastRP &[5pt] \\
            };
\end{tikzpicture}
\caption{Running time required per method (using 16-threads) to generate a 512-size node embedding per (a) number of vertices in the graph |V| and (b) number of undirected edges in the graph |E|; and (c) average running time percent increase compared to the 64-size node embedding baseline.}
\label{fig:running-times}
\end{figure}

==> tables/classification-macro.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{3.5pt}
\small
\centering{
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{S}{>{\hsize=.5\hsize}C}
\begin{tabularx}{\linewidth}{p{2cm}CCCCCC}
\emph{dataset} & PPI & BlogCatalog & CoCit & Flickr & YouTube & Orkut\\
    \midrule
DeepWalk & 12.89  \scriptsize{$\pm$ \emph{1.66}} & 18.69  \scriptsize{$\pm$ \emph{1.17}} & 26.96  \scriptsize{$\pm$ \emph{0.50}} & 13.42  \scriptsize{$\pm$ \emph{1.23}} & 31.11  \scriptsize{$\pm$ \emph{1.08}} & 85.86  \scriptsize{$\pm$ \emph{0.23}} \\
node2vec & 12.19  \scriptsize{$\pm$ \emph{2.34}} & 16.24  \scriptsize{$\pm$ \emph{1.11}} & 27.23  \scriptsize{$\pm$ \emph{0.38}} & 7.14  \scriptsize{$\pm$ \emph{0.20}}  & 25.03  \scriptsize{$\pm$ \emph{2.89}} & DNC                                  \\
VERSE & 9.54  \scriptsize{$\pm$ \emph{2.22}}  & 12.33  \scriptsize{$\pm$ \emph{1.58}} & 26.78  \scriptsize{$\pm$ \emph{1.58}} & 7.2  \scriptsize{$\pm$ \emph{1.28}}   & 27.16  \scriptsize{$\pm$ \emph{0.15}} & 79.34  \scriptsize{$\pm$ \emph{1.28}} \\
FastRP & 11.11  \scriptsize{$\pm$ \emph{1.20}} & 17.83  \scriptsize{$\pm$ \emph{1.90}} & 16.78  \scriptsize{$\pm$ \emph{1.49}} & 12.28  \scriptsize{$\pm$ \emph{2.72}} & 7.21  \scriptsize{$\pm$ \emph{0.20}}  & DNC                                   \\
\midrule
\thiswork & \textbf{13.04}  \scriptsize{$\pm$ \emph{1.06}} & 17.37  \scriptsize{$\pm$ \emph{0.97}} & \textbf{28.6}  \scriptsize{$\pm$ \emph{0.65}}  & 10.78  \scriptsize{$\pm$ \emph{1.20}} & 27.52  \scriptsize{$\pm$ \emph{1.60}} & 75.28  \scriptsize{$\pm$ \emph{1.20}} \\
\bottomrule
\end{tabularx}}
\caption{Macro-F1 classification.}
\label{tbl:exp-classification-macro}
\end{table}

==> tables/graph-statistics.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{3.5pt}
\small
\centering{
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{S}{>{\hsize=.5\hsize}C}
\caption{Dataset attributes: size of vertices $|V|$, edges $|E|$,  labels $|L|$, employed labeled vertices $|S|$}
\label{tbl:graph-statistics}
%\tiny
\begin{tabularx}{\linewidth}{p{2.5cm}RR@{}R@{}RC}
\toprule
Dataset & $|V|$ & $|E|$ & $|L|$ & $|S|$ & Source\\
\midrule
PPI & 3,890 & 38,292 & 40 & 3,890 & \cite{stark2006biogrid}\\
POS & 4,777 & 92,406 & 50 & 4,777 & \cite{mahoney2011wikipedia}\\
BlogCatalog & 10,312 & 333,983 & 39 & 10,312 & \cite{tang2010social}\\
MAG-CoCit & 44,034 & 195,361 & 15 & 44,034 & \cite{mag2016}\\
MAG-CoAuthor & 51,821 & 355,926 & --- & --- & \cite{mag2016}\\
Flickr & 80,513 & 5,899,882 & 195 & 80,513 & \cite{tang2010social}\\
YouTube & 1,138,499 & 2,990,443 & 47 & 31,703 & \cite{tang2010social}\\
Amazon2M & 2,449,029 & 61,859,076 & --- & --- & \cite{clustergcn}\\
Orkut & 3,072,441 & 117,185,083 & 50 & 109,695 & \cite{yang2015defining}\\
Friendster & 65,608,366 & 1,806,067,135 & --- & --- & \cite{yang2015defining}\\
\bottomrule
\end{tabularx}}

\end{table}
